On Transfer Learning of Traditional Frequency and Time Domain Features in Turning

There has been an increasing interest in leveraging machine learning tools for chatter prediction and diagnosis in discrete manufacturing processes. Some of the most common features for studying chatter include traditional signal processing tools such as Fast Fourier Transform (FFT), Power Spectral Density (PSD), and the Auto-correlation Function (ACF). In this study, we use these tools in a supervised learning setting to identify chatter in accelerometer signals obtained from a turning experiment. The experiment is performed using four different tool overhang lengths with varying cutting speed and the depth of cut. We then examine the resulting signals and tag them as either chatter or chatter-free. The tagged signals are then used to train a classifier. The classification methods include the most common algorithms: Support Vector Machine (SVM), Logistic Regression (LR), Random Forest (RF), and Gradient Boost (GB). Our results show that features extracted from the Fourier spectrum are the most informative when training a classifier and testing on data from the same cutting configuration yielding accuracy as high as %96. However, the accuracy drops significantly when training and testing on two different configurations with different structural eigenfrequencies. Thus, we conclude that while these traditional features can be highly tuned to a certain process, their transfer learning ability is limited. We also compare our results against two other methods with rising popularity in the literature: Wavelet Packet Transform (WPT) and Ensemble Empirical Mode Decomposition (EEMD). The latter two methods, especially EEMD, show better transfer learning capabilities for our dataset.

==> methods.tex <==

\section{Methods}
\label{sec:Methods}
In this section, we briefly describe how to extract chatter features by using traditional signal processing methods.
Fast Fourier Transform (FFT), Power Spectral Density(PSD) and auto-correlation function are methods widely used in signal processing. 


In this study, we used a feature vector composed from from three signal processing methods to detect chatter and compared their performance with the ones obtained from WPT/EEMD. 
Features for FFT, PSD and auto-correlation function are obtained by using the peaks. 
We started by using the both the $x$ and $y$ components of the first five peaks are used as features to train a classifier. 
Four different classifiers are utilized to compare signal processing based feature extraction methods to the WPT/EEMD. 
The results obtained using these classifiers for each cutting configuration are provided in Table~\ref{tab:FFT_PSD_ACF_Without_RFE}.

Table~\ref{tab:FFT_PSD_ACF_Without_RFE} shows that classifiers trained with the traditional signal processing features have an overfitting problem (significantly higher accuracy rates when training versus testing). 
Recursive feature elimination was used to solve this problem. 
Since we use the combinations of the ranked features, we decreased the total number of features for a signal by decreasing the number of peaks used in feature extraction from five to two.
Therefore, we have 12 features. 
These features are ranked and they are trained with four different classifiers.
We only report the best results obtained from the classifiers for each stickout case in Table~\ref{tab:FFT_PSD_ACF_With_RFE}.
These results are also compared to the ones obtained with WPT and EEMD in Fig.~\ref{fig:compare_WPT_EEMD_SPM}.

%------------------------------
\begin{figure*}[t]
\centering
\includegraphics[width=0.8\textwidth,height=.80\textheight,keepaspectratio]{Bar_Plot_Feature_Ranking_SVM_FFT_Based_Methods.png}
\caption{Bar plot for feature ranking obtained from SVM-RFE for 5.08 cm (2 inch) stickout case with FFT/PSD/ACF based method. ($f_{1},\ldots,f_{4}$), ($f_{4},\ldots,f_{8}$) and ($f_{9},\ldots,f_{12}$) belong to features obtained from peaks of FFT, PSD and ACF respectively.}
\label{fig:Feature_Ranking_Bar_Plot_SVM_FFT}
\end{figure*}
%------------------------------

We also compare the WPT and the EEMD with the feature extraction method based on FFT/PSD/ACF. 
It is seen that the FFT/PSD/ACF method has higher accuracies in Fig~.\ref{fig:compare_WPT_EEMD_SPM}. 
On the other hand, that same method has significantly lower accuracies with respect to WPT/EEMD in transfer learning (see Fig.~\ref{fig:comparison_high_acc_4_classifier_transfer_learning}). 
